Routes to turbulence in Taylor-Couette flow

Fluid flows between rotating concentric cylinders exhibit two distinct routes to turbulence. In flows dominated by inner-cylinder rotation, a sequence of linear instabilities leads to temporally chaotic dynamics as the rotation speed is increased. The resulting flow patterns occupy the whole system and sequentially lose spatial symmetry and coherence in the transition process. In flows dominated by outer-cylinder rotation, the transition is abrupt and leads directly to turbulent flow regions that compete with laminar ones. We here review the main features of these two routes to turbulence. Bifurcation theory rationalises the origin of temporal chaos in both cases. However, the catastrophic transition of flows dominated by outer-cylinder rotation can only be understood by accounting for the spatial proliferation of turbulent regions with a statistical approach. We stress the role of the rotation number (the ratio of Coriolis to inertial forces) and show that it determines the lower border for the existence of intermittent laminar-turbulent patterns.

==> userDefs/myCommands.tex <==
% to get your spacing straight
\RequirePackage{xspace}                           

\DeclareRobustCommand{\RBC}{Rayleigh--B\'enard convection\xspace}
\DeclareRobustCommand{\TCF}{Taylor--Couette flow\xspace}

% special math characters
\RequirePackage{siunitx}

\DeclareRobustCommand{\d}{\,d\!}                                                       % increment for integrals
\DeclareRobustCommand{\imag}{\ensuremath{\dot{\imath}}\xspace}                         % imaginary unit
\DeclareRobustCommand{\orderof}[1]{\ensuremath{\mathcal{O}\hspace{-0.1em}(\num{#1})}\xspace}   % magnitude
\DeclareRobustCommand{\real}{\ensuremath{\mathcal{R}}\xspace}                          % real part
\DeclareRobustCommand{\Bessel}{\ensuremath{\mathcal{J}_{0}}\xspace}                    % Bessel function

% statistical average delimiter
\DeclareRobustCommand{\lla}{\left\langle}
\DeclareRobustCommand{\rra}{\right\rangle}

% non-dimensional numbers
\DeclareRobustCommand{\Nusselt}{\ensuremath{N\hspace{-0.27em}u}\xspace} % Nusselt number
\DeclareRobustCommand{\Nui}{\ensuremath{N\hspace{-0.27em}u_i}\xspace}   % Nusselt number
\DeclareRobustCommand{\Nuo}{\ensuremath{N\hspace{-0.27em}u_o}\xspace}   % Nusselt number
\DeclareRobustCommand{\Rayleigh}{\ensuremath{R\hspace{-0.1em}a}\xspace} % Rayleigh number
\DeclareRobustCommand{\Reynolds}{\ensuremath{R\hspace{-0.1em}e}\xspace} % Reynolds number
\DeclareRobustCommand{\ReTau}{\ensuremath{R\hspace{-0.1em}e_{\tau}}\xspace}
\DeclareRobustCommand{\ROmega}{\ensuremath{R_{\Omega}}\xspace}          % rotation number
\DeclareRobustCommand{\ReS}{\ensuremath{R\hspace{-0.1em}e_{S}}\xspace}  % shear Reynolds number
\DeclareRobustCommand{\Rei}{\ensuremath{R\hspace{-0.1em}e_{i}}\xspace}  % inner Reynolds number
\DeclareRobustCommand{\Reo}{\ensuremath{R\hspace{-0.1em}e_{o}}\xspace}  % outer Reynolds number
\DeclareRobustCommand{\Taylor}{\ensuremath{T\hspace{-0.3em}a}\xspace}   % Taylor number
\DeclareRobustCommand{\rratio}{\ensuremath{\eta}\xspace}                % radaius ratio, not needed just eta?
\DeclareRobustCommand{\aspratio}{\ensuremath{\Gamma}\xspace}            % aspect ratio not needed, just Gamma?
\DeclareRobustCommand{\ri}{\ensuremath{r_i}\xspace}                     % Inner cylinder radius
\DeclareRobustCommand{\ro}{\ensuremath{r_o}\xspace}                     % Outer cylinder radius
\DeclareRobustCommand{\omegai}{\ensuremath{\Omega_i}\xspace}            % Inner cylinder angular velocity
\DeclareRobustCommand{\omegao}{\ensuremath{\Omega_o}\xspace}            %  Outer cylinder angular velocity
\DeclareRobustCommand{\gap}{\ensuremath{d}\xspace}                      % Gap width (i.e., r_o-r_i), not needed just d?
\DeclareRobustCommand{\visc}{\ensuremath{\nu}\xspace}                   % Fluid kinematic viscosity, not needed just \nu
\DeclareRobustCommand{\lifetime}{\ensuremath{\tau_{d}}\xspace}          % turbulence lifetime
\DeclareRobustCommand{\splittime}{\ensuremath{\tau_{s}}\xspace}         % turbulence lifetime
\DeclareRobustCommand{\torque}{\ensuremath{M}\xspace}                   % We use nusselt here?!?!?

% vector operators
\renewcommand{\vec}{\boldsymbol}
\DeclareRobustCommand{\divergence}{\operatorname{div}}
\DeclareRobustCommand{\gradient}{\operatorname{grad}}
\RequirePackage{rotating} % provides sideways
\DeclareRobustCommand{\laplacian}{\vec{\Delta}}
\renewcommand{\nabla}{\begin{sideways}\begin{sideways}$\laplacian$\end{sideways}\end{sideways}}

% relations
\DeclareRobustCommand{\constraint}{\stackrel{!}{=}}

% some software names
\RequirePackage{xspace}
\RequirePackage{hyperref}
\DeclareRobustCommand{\code}[1]{\textbf{\texttt{\color{black}#1}}\xspace}
\DeclareRobustCommand{\hdf}{\href{https://en.wikipedia.org/wiki/Hierarchical_Data_Format}{\code{HDF5}}\xspace}
\DeclareRobustCommand{\mpi}{\href{https://en.wikipedia.org/wiki/Message_Passing_Interface}{\code{MPI}}\xspace}
\DeclareRobustCommand{\nsc}{\href{https://github.com/dfeldmann/nsCouette}{\code{nsCouette}}\xspace}
\DeclareRobustCommand{\tlab}{\href{https://github.com/turbulencia/Tlab}{\code{tLab}}\xspace}
\DeclareRobustCommand{\omp}{\href{https://en.wikipedia.org/wiki/OpenMP}{\code{OpenMP}}\xspace}
\DeclareRobustCommand{\python}{\href{https://www.python.org/}{\code{Python}}\xspace}
\DeclareRobustCommand{\pangaea}{\href{https://www.pangaea.de}{\textbf{\texttt{Pangaea}}}\xspace}

% common abbreviations
\DeclareRobustCommand{\ie}{i.\,e.\,}
\DeclareRobustCommand{\Ie}{I.\,e.\,}
\DeclareRobustCommand{\eg}{e.\,g.\,}
\DeclareRobustCommand{\Eg}{E.\,g.\,}
\DeclareRobustCommand{\etc}{etc.}
\DeclareRobustCommand{\etal}{\textit{et al.}}

% draft stage
% \DeclareRobustCommand{\mod}[1]{{\color{Vermillion}#1}} % \xspace
\DeclareRobustCommand{\mod}[1]{{\color{Black}#1}} % \xspace
\DeclareRobustCommand{\df}[1]{{\color{Vermillion}(\textbf{Feldi}: \textit{#1})}\xspace}
\DeclareRobustCommand{\ma}[1]{{\color{Vermillion}(\textbf{Marc}: \textit{#1})}\xspace}
\DeclareRobustCommand{\ka}[1]{{\color{Vermillion}(\textbf{Kerstin}: \textit{#1})}\xspace}
\DeclareRobustCommand{\mb}[1]{{\color{Vermillion}(\textbf{Michael}: \textit{#1})}\xspace}
\DeclareRobustCommand{\db}[1]{{\color{Vermillion}(\textbf{Daniel~B}: \textit{#1})}\xspace}
\DeclareRobustCommand{\todo}[1]{{\color{Vermillion}(\textbf{To do}: \textit{#1})}\xspace}
\DeclareRobustCommand{\q}[1]{{\color{Vermillion}(\textbf{Question}: \textit{#1})}\xspace}
\DeclareRobustCommand{\tentative}[1]{{\color{Vermillion}#1}}
\DeclareRobustCommand{\Editor}{\item[{\color{Vermillion}Edit.}]\color{Grey}}
\DeclareRobustCommand{\RefereeA}{\item[{\color{Vermillion}Ref. A}]\color{Grey}}
\DeclareRobustCommand{\RefereeB}{\item[{\color{Vermillion}Ref. B}]\color{Grey}}
\DeclareRobustCommand{\Response}{\item[{\color{Blue}Resp.}]\color{Black}}


==> userDefs/myPreamble.tex <==
% font encoding
\usepackage[T1]{fontenc}    % output
\usepackage[utf8]{inputenc} % input
\RequirePackage{url}        % to avoid probs with special chars in email or web address

% language settings
\usepackage[UKenglish]{babel}

% math, units and numbers
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amstext}
\RequirePackage{dsfont}
\RequirePackage{siunitx}
\PassOptionsToPackage{decimalsymbol=.}{siunitx}
\sisetup{tight-spacing=true}
%\sisetup{print-unity-mantissa=false}

% \RequirePackage{xfrac}

% figures
\RequirePackage{graphicx}
\RequirePackage{overpic}
\RequirePackage{epsfig}
\RequirePackage{float}
\RequirePackage{animate}

% tables
\RequirePackage{array}
\RequirePackage{longtable, lscape}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{booktabs}

% make it gay
\RequirePackage{color}
\definecolor{Orange}{cmyk}{0, 0.5, 1, 0} % appropriate set for colour-blind
\definecolor{SkyBlue}{cmyk}{0.8, 0, 0, 0}
\definecolor{BluishGreen}{cmyk}{0.97, 0, 0.75, 0}
\definecolor{Yellow}{cmyk}{0.1, 0.05, 0.9, 0}
\definecolor{Blue}{cmyk}{1, 0.5, 0, 0}
\definecolor{Vermillion}{cmyk}{0, 0.8, 1, 0}
\definecolor{ReddishPurple}{cmyk}{0.1, 0.7, 0, 0}
\definecolor{Grey}{cmyk}{0, 0, 0, 0.6}
\definecolor{Black}{cmyk}{0, 0, 0, 1}

% pdf hyperref functionality
\RequirePackage{hyperref}
\hypersetup{colorlinks=true, linkcolor=Blue, urlcolor=Blue, citecolor=Blue}

% draft stage only
% \usepackage[export]{adjustbox}
% \RequirePackage{printlen}
% \RequirePackage{layouts}
% \RequirePackage{blindtext}
% \RequirePackage{lineno}

